Supervised and Unsupervised Ensembling for Knowledge Base Population

We present results on combining supervised and unsupervised methods to ensemble multiple systems for two popular Knowledge Base Population (KBP) tasks, Cold Start Slot Filling (CSSF) and Tri-lingual Entity Discovery and Linking (TEDL). We demonstrate that our combined system along with auxiliary features outperforms the best performing system for both tasks in the 2015 competition, several ensembling baselines, as well as the state-of-the-art stacking approach to ensembling KBP systems. The success of our technique on two different and challenging problems demonstrates the power and generality of our combined approach to ensembling.

==> 2015/abstract.tex <==
We present results on using stacking to ensemble multiple systems for the
Knowledge Base Population English Slot Filling (KBP-ESF) task.  In addition to
using the output and confidence of each system as input to the stacked
classifier, we also use features capturing how well the systems agree about the
provenance of the information they extract.  We demonstrate that our stacking
approach outperforms the best system from the 2014 KBP-ESF competition as well
as alternative ensembling methods employed in the 2014 KBP Slot Filler
Validation task and several other ensembling baselines.  Additionally, we
demonstrate that including provenance information further increases the
performance of stacking.


==> 2015/acknowledgement.tex <==
We thank the anonymous reviewers for their valuable feedback. This research was supported in part by the DARPA DEFT program under AFRL grant FA8750-13-2-0026 and by MURI ARO grant W911NF-08-1-0242.

==> 2015/background.tex <==
For the past few years, the Text Analysis Conference (TAC) has been
conducting the English Slot Filling (ESF) Task in the Knowledge Base
Population (KBP) track among various other
tasks \cite{surdeanu:tac13,surdeanu:tac14}. In the ESF task, the goal
is to fill specific slots of information for a given set of query entities
(of type person or organization) from a supplied text corpus.
%% This has
%% promoted the development of various ESF systems that employ different
%% methodologies to perform slot filling.
The participating systems
employ a variety of techniques in different stages of the slot filling
pipeline such as entity search, relevant document extraction, relation
modeling and inferencing. In 2014, the top performing system {\it
DeepDive with Expert Advice} from Stanford
University \cite{wazalwar:tac14} employed distant
supervision \cite{mintz:acl09} and Markov Logic
Networks \cite{domingos:bkchapter08} in their learning and inferencing
system. Another system, {\it RPI\_BLENDER} \cite{hong:tac14}, used a
restricted fuzzy matching technique in a framework that learns event
triggers and employs them to extract relations from documents.
%% We used {\it LSV} \cite{roth:tac13} which was the best
%% performing system in 2013 as our base relation extraction system and
%% coupled it with inferencing algorithms based on Bayesian Logic
%% Programs (BLP) \cite{raghavan:acl12}.

Given the diverse set of slot-filling systems available, it is
interesting to explore methods for ensembling these systems. In this
regard, TAC also conducts a Slot Filler Validation (SFV) task where
the goal is to improve the slot-filling performance using the output
of existing systems. The input for this task is the set of outputs
from all slot-filling systems and the expected output is a filtered
set of slot fills. As with the basic task, participating systems
employ a variety of techniques to perform validation. For instance,
{\it RPI\_BLENDER} uses a Multi-dimensional Truth Finding
model \cite{yu:coling14} which is an unsupervised validation approach
based on computing multidimensional credibility scores. Also, the {\it
UI\_CCG} system \cite{sammons:tac14} develops two different validation
systems using entailment and majority voting.

However, {\it stacking} \cite{sigletos:jmlr05,wolpert:nn92} has not
previously been employed for ensembling KBP-ESF systems. In
stacking, a meta-classifier is learned from the output of multiple
underlying systems. In our work, we translate this to the context of
ensembling slot filling systems and build a {\it stacked
meta-classifier} that learns to combine the results from individual
slot filling systems. We detail our stacking approach for ensembling
existing slot filling systems in Section 4.


==> 2015/conclusion.tex <==
This paper has presented experimental results showing that {\it
stacking} is a very promising approach to ensembling KBP systems. From
our literature survey, we observe that we are the first to employ
stacking and combine it with provenance information to ensemble KBP
systems. Our stacked meta-classifier provides an F1 score of 50.1\% on
2014 KBP ESF, outperforming the best ESF and SFV systems from the 2014
competition, and thereby achieving a new state-of-the-art for this
task.  We found that provenance features increased accuracy,
highlighting the importance of provenance information (even without
accessing the source corpus) in addition to confidence scores for
ensembling information extraction systems. 
%In this work, we have
%utilized only filler provenance information. 

%In the future, we plan to
%investigate the use of relation provenance and add additional features
%to enhance the performance of our stacked ensembles.


==> 2015/experimental_evaluation.tex <==
\section{Experimental Evaluation}
\label{section:exp}

\begin{figure*}[!ht]
\centering
\begin{tabular}{cc}
\includegraphics[width=68mm]{plots/pr-majority-10.png} & \includegraphics[width=68mm]{plots/pr-majority.png}\\
Common systems dataset & All 2014 SFV systems dataset\\
\end{tabular}
\caption{Precision-Recall curves for identifying the best voting performance on the two datasets}
\label{figure:pr}
\end{figure*}

This section describes a comprehensive set of experiments evaluating
ensembling for the KBP ESF task.  Our experiments are divided into two
subsets based on the datasets they employ. Since our stacking
approach relies on 2013 SFV data for training, we build a dataset of
one run for every team that participated in {\it both} the 2013 and 2014
competitions and call it the \emph{common systems dataset}. There are $10$ common teams of the $17$ teams that participated in ESF 2014. The other dataset comprises of all 2014 SFV systems (including all runs of all $17$ teams that participated in 2014). There are $10$ systems in the common systems dataset, while there are $65$ systems in the all 2014 SFV dataset. Table~\ref{table:common} gives a list of the common systems for 2013 and 2014 ESF task.

\begin{table}[!ht]
\centering
\begin{tabular}{| c |}
\hline
\textbf{Common Systems}\\
\hline
LSV\\
IIRG\\
UMass\_IESL\\
Stanford\\
BUPT\_PRIS\\
RPI\_BLENDER\\
CMUML\\
NYU\\
Compreno\\
UWashington\\
\hline
\end{tabular}
\caption{Common teams for 2013 and 2014 ESF}
\label{table:common}
\end{table}

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{plots/pipeline-new.png}
\caption{Our system pipeline for evaluating supervised ensembling approaches}
\label{fig:pipeline}
\end{figure*}

\begin{table*}[!ht]
\centering
\begin{tabular}{| c | c | c | c | }
\hline
\textbf{Baseline} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
 \hline
 \hline
 Union  &0.067	&\textbf{0.762}	&0.122\\
 %Intersection &\textbf{1.0}&	0.001&	0.002\\
Voting (threshold learned on 2013 data)&\textbf{ 0.641}&0.288&	0.397\\
Voting (optimal threshold for 2014 data)& 0.547&0.376&\textbf{0.445}\\
\hline
\end{tabular}
\caption{Performance of baselines on all 2014 SFV dataset (65 systems)}
\label{table:results2}
\end{table*}

\begin{table*}[!ht]
\centering
\begin{tabular}{| c | c | c | c | }
\hline
\textbf{Approach} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
 \hline
 \hline
 Union  &0.176 &	\textbf{0.647}&	0.277\\
% Intersection &\textbf{1.0}&	0.003	&0.006\\
Voting (threshold learned on 2013 data)&\textbf{0.694}&0.256&0.374\\
 Best ESF system in 2014 (Stanford) &0.585&	0.298 &	0.395\\
Voting (optimal threshold for 2014 data) & 0.507	& 0.383	& 0.436\\
Stacking &0.606	&0.402&	0.483\\
Stacking + Relation &0.607&0.406&	0.486\\
Stacking +  Provenance (document)&0.499	&0.486&	0.492\\
Stacking +  Provenance (document) + Relation&0.653	&0.400	&0.496\\
Stacking +  Provenance (document and offset) + Relation&0.541	&0.466	&\textbf{0.501}\\
\hline
\end{tabular}
\caption{Performance on the common systems dataset (10 systems) for various configurations. All approaches except the Stanford system are our implementations.}
\label{table:results1}
\end{table*}

\subsection{Methodology and Results}

For our unsupervised ensembling baselines, we evaluate on both the
common systems dataset as well as the entire 2014 SFV dataset. We
compare our stacking approach to three unsupervised baselines. The first
is {\it Union} which takes the combination of values for all systems
to maximize recall.  If the slot type is list-valued, it classifies all slot
fillers as correct and always includes them. If the slot type is
single-valued, if only one systems attempts to answer it, then it
includes that system's slot fill else if multiple systems attempt,
then it only includes the slot fill with the highest confidence value
as correct and discards the rest.
%The second baseline is {\it Intersection}, which attempts to maximize precision. For a given query and slot, if the slot type is list, it takes the intersection of the sets of values produced by each of the systems.  If the slot type is single-valued, it classifies the slot fill as correct if only if all the systems agree on the value.

The second baseline is {\it Voting}.  For this approach, we vary the
threshold on the number of systems that must agree on a slot-fill from
one to all. This gradually changes the system from the union to
intersection of the slot fills, and we identify the threshold that
results in the highest F1 score. We learn a threshold on the 2013 SFV
dataset (containing 52 systems) that results in the best F1 score,
thereafter, we use this threshold for the voting baseline on 2014 SFV
dataset. We do the same thing we did for 2013 dataset for the common
systems dataset. We learn a threshold on the 2013 common systems that results in the best F1 score and use this threshold  for the voting baseline on 2014 common systems.

The third baseline is an ``oracle threshold'' version of {\it
  Voting}. Since the best threshold for 2013 may not
necessarily be the best threshold for 2014, we identify the best
threshold for 2014 by plotting a Precision-Recall curve and finding the best
F1 score for the voting baseline on both the SFV and common systems datasets.  Figure~\ref{figure:pr} shows the
Precision-Recall curve for two datasets for finding the best
possible F1 score using the voting baseline. We find that for the
common systems dataset, a threshold of $3$ (of $10$) systems gives the
best F1 score, while for the all 2014 SFV dataset, a threshold of $10$
(of $65$) systems gives the highest F1.  Note that this gives an
upper-bound on the best results that can be achieved with voting,
assuming an optimal threshold is chosen. Since the upper-bound could
not be predicted without using the 2014 dataset, this baseline has an
unfair advantage.  Table~\ref{table:results2} shows the performance of
all $3$ baselines on the all 2014 SFV systems dataset.

For all our supervised ensembling approaches, we train on the 2013 SFV
data and test on the 2014 data for the common systems. We have $5$
different supervised approaches. Our first approach is stacking the
common systems using their confidence scores to learn a classifier. As
discussed earlier, in stacking we train a meta-classifier that
combines the systems using their confidence scores as features. Since
the common systems dataset has $10$ systems, this classifier uses $10$
features. The second approach also provides stacking with a nominal
feature giving the relation name (as listed in
Table~\ref{table:slot_types}) for the given slot instance.  This
allows the system to learn different evidence-combining functions for
different slots if the classifier finds this useful.  For our
third approach, we also give stacking the document provenance feature
described in Section~\ref{sec:algo}.  Altogether this approach has
$11$ features ($10$ confidence score + $1$ document provenance
score). The fourth approach uses confidences, the document provenance
feature, and a nominal feature giving the relation name for the slot
instance. Our final approach also includes the offset provenance (OP)
feature discussed in Section~\ref{sec:algo}.  There are altogether
$13$ features in this approach. All our supervised approaches use the
Weka package \cite{hall:kdd09} for training the meta-classifier, using an
L1-regularized SVM with a linear kernel (other classifiers gave
similar results).  Figure~\ref{fig:pipeline} shows our system pipeline
for evaluating supervised ensembling
approaches. Table~\ref{table:results1} gives the performance of all
our supervised approaches as well as our unsupervised baselines for
the common systems dataset.

\vspace{0.5cm}
Analysis by \newcite{surdeanu:tac14} suggests that 2014 ESF queries are
more difficult than those for 2013. They compare several common
systems for both years and find there is a considerable drop in their
performance. Thus, in order to have a better understanding of our
results, we plot a learning curve by training on different sizes of
the 2013 SFV data and using the scorer to measure the F1 score on the
2014 SFV data for the $10$ common systems.
Figure~\ref{figure:learning} shows the learning curve thus
obtained. Although there are certain proportions of the dataset when
the F1 score drops which we suspect is due to overfitting the 2013
data, there is still a strong correlation between the 2013 training
data size and F1 score on the 2014 dataset. Thus we can infer that
training on 2013 data is useful even though the 2013 and 2014 data are
fairly different. Although the queries change, the common systems
remain more-or-less the same and stacking enables a meta-classifier to
weigh those common systems based on their 2013 performance.

\begin{figure}[!ht]
\centering
\includegraphics[width=68mm]{plots/learning-f1.png}
\caption{Learning curve for training on 2013 and testing on 2014 common systems dataset}
\label{figure:learning}
\end{figure}

To further validate our approach, we divide the 2013 SFV data based on the systems that extracted those slot fills. Then we sort the systems, from higher to lower, based on the number of false positives produced by them in the ensembling approach.  Thereafter we train a classifier in an incremental fashion adding one system's slot fills for training at each step and analyzing the performance on 2014 data. This allows us to analyze the results at the system level. Figure~\ref{figure:incremental} shows the plot of F1 score vs. the number of systems at each step. The figure shows huge improvement in F1 score at steps $6$ and $7$. At step $6$ the Stanford system is added to the pool of systems which is the best performing ESF system in 2014 and fourth best in 2013. At step $7$ the UMass system is added to the pool and although the system on it own is weak, it boosts the performance of our ensembling approach. This is because the UMass system alone contributes approximately $24\%$ of the 2013 training data. Thus adding this one system significantly improves the training step leading to better performance. We also notice that our system becomes less conservative at this step and we suspect the reason for this is the way they calculate their confidence scores. The UMass system uses matrix factorization and the confidence values that we use for our training are obtained by applying logistic function to the factorization score \cite{singh:tac2013}. The UMass system thus enables our meta-classifier to have a higher recall for small decrease in precision and thus boosting the overall F1 measure. Without it, the classifier produces high precision but low recall and decreases the overall F1 score by approximately $6$ points.

\begin{figure}[!ht]
\centering
\includegraphics[width=68mm]{plots/incremental.png}
\caption{Incrementally training on 2013 by adding a system at each step and testing on 2014 common systems dataset}
\label{figure:incremental}
\end{figure}

We also experimented with cross validation within the 2014 dataset in order to make our results even stronger. Since we used only 2014 data for this experiment we also included the relation provenance as discussed in Section~\ref{sec:provenance}. Table~\ref{table:results_cv} shows the results on 10-fold cross-validation on 2014 data with only the filler provenance and with both the filler and relation provenance. The performance of using only the filler provenance is slightly worse than training on 2013 because the 2014 SFV data has many fewer instances but uses more systems for learning compared to the 2013 SFV data.

\begin{table*}[!ht]
\centering
%\begin{tabular}{|p{3cm}|p{1cm}|p{1cm}|p{1cm}|}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Approach} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
 \hline
 \hline
Stacking + Filler provenance + Relation&0.606&	0.415 &	0.493\\
Stacking +  Filler and Relation provenance + Relation &\textbf{0.609} & \textbf{0.434} &\textbf{0.506}\\
\hline
\end{tabular}
\caption{10-fold Cross-Validation on 2014 SFV dataset(65 systems)}
\label{table:results_cv}
\end{table*}

\begin{table*}[!ht]
\centering
%\begin{tabular}{|p{3cm}|p{1cm}|p{1cm}|p{1cm}|}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Baseline} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
 \hline
 \hline
 Union  &0.054	&\textbf{0.877}	& 0.101\\
 %Intersection &\textbf{1.0}	&0.001	&0.003\\
Voting (threshold learned on 2013 data)&\textbf{0.637}&0.406&0.496\\
Voting (optimal threshold for 2014 data)&0.539	&0.526&	\textbf{0.533}\\
\hline
\end{tabular}
\caption{Baseline performance on all 2014 SFV dataset (65 systems) using unofficial scorer}
\label{table:results4}
\end{table*}

\begin{table*}[!ht]
\centering
\begin{tabular}{| c | c | c | c | }
\hline
\textbf{Approach} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
 \hline
 \hline
Union  &0.177&\textbf{0.922}	&0.296\\
 %Intersection &\textbf{1.0}&	0.003	&0.006\\
Voting (threshold learned on 2013 data)&\textbf{0.694}&0.256&0.374\\
Best published SFV result in 2014 (UIUC) &0.457 &0.507	 &0.481	\\
Voting (optimal threshold for 2014 data) & 0.507	& 0.543 &	0.525\\
Stacking +  Provenance(document)&0.498	&0.688&	0.578\\
Stacking &0.613&	0.562	&0.586\\
Stacking + Relation &0.613&0.567&0.589\\
Stacking +  Provenance(document and offset)+ Relation&0.541&	0.661	&0.595\\
Stacking +  Provenance(document)+ Relation&0.659	&0.56	&\textbf{0.606}\\
\hline
\end{tabular}
\caption{Performance on the common systems dataset (10 systems) for various configurations using the unofficial scorer. All approaches except the UIUC system are our implementations.}
\label{table:results3}
\end{table*}

The TAC KBP official scoring key for the ESF task includes human annotated slot
fills along with the pooled slot fills obtained by all participating
systems. However, \newcite{sammons:tac14} use an unofficial scoring key in their
paper that does not include human annotated slot fills. In order to compare to
their results, we also present results using the same unofficial key.
Table~\ref{table:results4} gives the performance of our baseline systems on the
2014 SFV dataset using the unofficial key for scoring. We note that our union
does not produce a recall of $1.0$ on the unofficial scorer due to our single-valued
slot selection strategy for multiple systems. As discussed earlier for the single-valued
slot, we include the slot fill with highest confidence (may not necessarily be correct) and
thus may not match the unofficial scorer.

Table~\ref{table:results3} gives the performance of all our supervised
approaches along with the baselines on the common systems dataset using the
unofficial key for scoring. UIUC is one of the two teams participating in the SFV
2014 task and the only team to report results, but they report $6$ different system
configurations and we show their best performance.

\subsection{Discussion}
Our results indicate that stacking with provenance information and relation
type gives the best performance using both the official ESF scorer as well as
the unofficial scorer that excludes the human-generated slot fills. Our
stacking approach that uses the 10 systems common between 2013 and 2014 also
outperforms the ensembling baselines that have the advantage of using {\it all
65} of the 2014 systems.  Our stacking approach would presumably perform even
better if we had access to 2013 training data for all 2014 systems.

Of course, the best-performing ESF system for 2014 did not have access to the
pooled slot fills of all participating systems. Although pooling the results
has an advantage, naive pooling methods such as the ensembling baselines, in
particular the voting approach, do not perform as well as our stacked
ensembles. Our best approach beats the best baseline for both the datasets by at
least $6$ F1 points using both the official and unofficial scorer.

As expected the {\it Union} baseline has the highest recall.  Among
the supervised approaches, stacking with document provenance produces
the highest precision and is significantly higher (approximately
$5\%$) than the approach that produces the second highest
precision. As discussed earlier, we also scored our approaches on the
unofficial scorer so that we can compare our results to the UIUC
system that was the best performer in the 2014 SFV task. Our best
approach beats their best system configuration by a F1 score of $12$
points. Our stacking approach also outperforms them on precision and
recall by a large margin.



==> 2015/introduction.tex <==
Using {\it ensembles} of multiple systems is a standard approach to improving
accuracy in machine learning \cite{dietterich:bkchapter00}. Ensembles have been
applied to a wide variety of problems in natural language processing, including
parsing \cite{henderson:emnlp99}, word sense disambiguation
\cite{pedersen:naacl00}, and sentiment analysis
\cite{whitehead:bkchapter10}.
This paper presents a detailed study of ensembling methods for the TAC {\it
Knowledge Base Population} (KBP) {\it English Slot Filling} (ESF)
task \cite{surdeanu:tac13,surdeanu:tac14}.

We demonstrate new state-of-the-art results on this KBP task using
{\it stacking} \cite{wolpert:nn92}, which trains a final
classifier to optimally combine the results of multiple systems.  We
present results for stacking all systems that competed in both the
2013 and 2014 KBP-ESF tracks, training on 2013 data and testing
on 2014 data.  The resulting stacked ensemble outperforms all systems
in the 2014 competition, obtaining an F1 of $48.6\%$ compared to $39.5\%$ for the
best performing system in the most recent competition.

Although the associated KBP Slot Filler Validation (SFV)
Track \cite{wang:tac13,yu:coling14,sammons:tac14} is officially focused on
improving the precision of individual existing systems by filtering
their results, frequently participants in this track also combine the
results of multiple systems and also report increased recall through
this use of ensembling.  However, SFV participants have not employed
stacking, and we demonstrate that our stacking approach outperforms
existing SFV ensembling systems.

KBP ESF systems must also provide {\it provenance} information, each
extracted slot-filler must include a pointer to a document passage
that supports it \cite{surdeanu:tac14}.  Some SFV
systems have used this provenance information to help filter and
combine extractions \cite{sammons:tac14}. Therefore, we also explored
enhancing our stacking approach by including additional input features
that capture provenance information. By including features that
quantify how much the ensembled systems agree on provenance, we
further improved our F1 score for the 2014 ESF task to $50.1\%$.

The remainder of the paper is organized as follows. Section 2 provides
background information on existing KBP-ESF systems and stacking.
Section 3 provides general background on the KBP-ESF task.  Section 4
describes our stacking approach, including how provenance information
is exploited. Section 5 presents comprehensive experiments comparing
this approach to existing results and several additional baselines,
demonstrating new state-of-the-art results on KBP-ESF. Section 6
reviews prior related work on ensembling for information extraction.
Section 7 presents our final conclusions and proposed directions for
future research.


==> 2015/problem_definition_and_algorithm.tex <==
%% In this section, we first provide an outline of TAC KBP English Slot Filling Task followed by the  definition of the problem of ensembling relation extractors for KBP Slot Filling Task. We then describe our Stacking algorithm in detail.

\section{Overview of KBP Slot Filling Task}
% Comment by Vidh
% Some of this section can be moved to experiments if needed
% putting content here tentatively till we get into some shape

\begin{table*}[!ht]
\centering
\small
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{2}{|c}{\textbf{Person}}                  &\multicolumn{2}{c|} {\textbf{Organization}   }              \\
\hline
per:alternate\_names  &per:cause\_of\_death & org:country\_of\_headquarters & org:founded\_by                 \\
per:date\_of\_birth      &per:countries\_of\_residence    & org:stateorprovince\_of\_headquarters &  org:date\_dissolved \\
per:age &per:statesorprovinces\_of\_residence & org:city\_of\_headquarters &org:website            \\
per:parents    &per:cities\_of\_residence            & org:shareholders  &org:date\_founded     \\
per:spouse  &per:schools\_attended                & org:top\_members\_employees      & org:members                           \\
per:city\_of\_birth   &per:city\_of\_death                  & org:political\_religious\_affiliation              & org:member\_of                        \\
per:origin            &per:stateorprovince\_of\_death       &org:number\_of\_employees\_members                & org:subsidiaries                      \\
per:other\_family   &per:country\_of\_death               & org:alternate\_names          & org:parents                           \\
per:title                            &    per:employee\_or\_member\_of         &&                                   \\
per:religion                         &        per:stateorprovince\_of\_birth                           &    &                               \\
per:children                         &       per:country\_of\_birth                         &        &                               \\
per:siblings                         &    per:date\_of\_death                    & &                                   \\
per:charges                          &             &&                          \\
\hline
\end{tabular}
\caption{Slots for PER and ORG queries}
\label{table:slot_types}
\end{table*}


The goal of the TAC KBP-ESF task \cite{surdeanu:tac13,surdeanu:tac14}
is to collect information (fills) about specific attributes (slots)
for a set of entities (queries) from a given corpus. The queries vary
in each year of the task and can be either a person (PER) or an
organization (ORG) entity. The slots are fixed and are listed in Table
\ref{table:slot_types} by entity type. Some slots (like per:age) are
{\it single-valued} while others (like per:children) are {\it list-valued} i.e., they
can take multiple slot fillers.

\subsection{Input and Output}

The input for the task is a set of queries and the corpus in which to
look for information. The queries are provided in XML format
containing basic information including an ID for the query, the name
of the entity, and the type of entity (PER or ORG). The corpus consists of
documents in XML format from discussion forums, newswire and the
Internet. Each document is identified by a unique document ID.

%include a sample query here ?

The output for the task is a set of slot fills for each input query.
Depending on the type, each query should have one line of output for
each of the corresponding slots containing the slot fill or a {\it
  NIL} filler. The output line for each slot fill contains the fields
shown in Table \ref{table:slotfill_output}. The query ID in Column 1
should match the ID of the query given as input. The slot name (Column
2) is one of the slots listed in Table \ref{table:slot_types} based on
entity type. Run ID (Column 3) is a unique identifier for each
system. Column 4 contains a {\it NIL} filler if the system could not
find any relevant slot filler. Otherwise, it contains the {\it
  relation provenance}. Provenance is of the form {\it
  docid:startoffset-endoffset}, where {\it docid} specifies a source
document from the corpus and the offsets demarcate the text in this
document supporting the relation.  The offsets correspond to the
span of the candidate document that describe the relation between
the query entity and the extracted slot filler.  Column 5 contains the
extracted slot filler. Column 6 is a filler provenance that is similar
in format to relation provenance but in this case the offset
corresponds to the portion of the document containing the
extracted filler. Column 7 is a confidence score which systems
can provide to indicate their certainty in the extracted information.

\subsection{Scoring}
The scoring for the ESF task is carried out as follows. The responses
from all slot-filling systems are pooled and a {\it key file} is
generated by having human assessors judge the correctness of these
responses. In addition, LDC includes a manual key of fillers
that were determined by human judges. Using the union of these keys as
the gold standard, precision, recall, and F1 scores are computed.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Column} & \textbf{Field Description} \\ \hline
Column 1        & Query ID                   \\ \hline
Column 2        & Slot name                  \\ \hline
Column 3        & Run ID                     \\ \hline
Column 4        & NIL or Relation Provenance \\ \hline
Column 5        & Slot filler                \\ \hline
Column 6        & Filler Provenance          \\ \hline
Column 7        & Confidence score           \\ \hline
\end{tabular}
\caption{SF Output line fields}
\label{table:slotfill_output}
\end{table}

\section{Ensembling Slot-Filling Systems}

Given a set of query entities and a fixed set of slots, the goal of
ensembling is to effectively combine the output of different
slot-filling systems.  As input, it takes the output of individual
systems (in the format described in previous section) containing slot
fillers and additional information such as provenance and confidence
scores. The output of the ensembling system is similar to the output
of an individual system, but it productively aggregates the slot
fillers from different systems.

\subsection{Algorithm}
\label{sec:algo}

This section describes our ensembling approach which trains a final
binary classifier using features that help judge the reliability and
thus correctness of individual slot fills.  In a final
{\it post-processing} step, the slot fills that get classified as
``correct" by the classifier are kept while the others are set to NIL.

\subsubsection{Stacking}

Stacking is a popular ensembling methodology in machine learning
\cite{wolpert:nn92} and has been very successful in many applications
including the top performing systems in the Netflix competition
\cite{sill:2009}. The idea is to employ multiple learners and combine
their predictions by training a ``meta-classifier'' to weight and
combine multiple models using their confidence scores as features.  By
training on a set of supervised data that is disjoint from that used
to train the individual models, it learns how to combine
their results into an improved ensemble model. We employ a single
classifier to train and test on all slot types using an L1-regularized
SVM with a linear kernel \cite{fan:ref08}.

\subsubsection{Using Provenance}
\label{sec:provenance}
As discussed above, each system provides provenance information for every non-
NIL slot filler. There are two kinds of provenance provided, the relation
provenance and the filler provenance. In our algorithm, we only use the filler
provenance for a given slot fill. This is because of the changes in the output
formats for the ESF task from 2013 to 2014. Specifically, the 2013 format is
comprised of three provenances namely filler, entity and justification while 2014
format has only two provenances namely filler and relation provenance. Hence,
we use the filler provenance that is common between 2013 and 2014 formats.
As described earlier, every provenance has a \emph{docid} and \emph{startoffset-endoffset}
that gives information about the document and offset in the document 
from where the slot fill has been extracted. In their SFV system, 
\newcite{sammons:tac14} effectively use this provenance information to 
help validate and filter slot fillers.  This motivated us to use provenance 
in our stacking approach as additional features as input to the meta-classifier.

We use provenance in two ways, first using the \emph{docid}
information, and second using the \emph{offset} information. We use
the docids to define a document-based provenance score in the following
way: for a given query and slot, if $N$ systems provide answers and a
maximum of $n$ of those systems give the same \emph{docid} in their
filler provenance, then the document provenance score for those $n$
slot fills is $n/N$. Similarly, other slot fills are given lower
scores based on the fraction of systems whose provenance document
agrees with theirs.  Since this provenance score is weighted by the
number of systems that refer to the same provenance, it measures the
reliability of a slot fill based on the document from where it was
extracted.

Our second provenance measure uses \emph{offsets}.  The degree of
overlap among the various system's offsets can also be a good
indicator of the reliability of the slot fill. The Jaccard similarity
coefficient is a statistical measure of similarity between sets and is
thus useful in measuring the degree of overlap among the offsets of
systems. %% The start and end offsets provided by the system is a range
%% and can thus serve as indicators of an overlap among the systems.
Slot fills have variable lengths and thus the provenance offset ranges
are variable too. A metric such as the Jaccard coefficient captures
the overlapping offsets along with normalizing based on the union and
thus resolving the problem with variable offset ranges. For a given
query and slot, if $N$ systems that attempt to answer it have the same \emph{docid} for their document provenance, then the offset provenance (OP) score for a slot fill by a system $x$ is calculated as
follows:

%\begin{small}
\[OP(x)=\frac{1}{|N|}\times\sum_{i\in N,i\neq x}^{}\frac{|\textsf{offsets(i)}\cap \textsf{offsets(x)}|}{|\textsf{offsets(i)}\cup \textsf{offsets(x)}|}\]
%\end{small}

Per our definition,  systems that extract slot fills from
\emph{different} documents for the same query slot have zero
overlap among offsets. We note that the offset provenance is always
used along with the document provenance and thus useful in
discriminating slot fills extracted from a different document for the
same query slot.  Like the document provenance score, the offset
provenance score is also a weighted feature and is a measure of
reliability of a slot fill based on the offsets in the document from
where it is extracted.  Unlike past SFV systems that use provenance
for validation, our approach does not need access to the large corpus
of documents from where the slot fills are extracted and is thus very
computationally inexpensive.

%% Since
%% the offset provenance score does not carry any information about the
%% document, it is used along with the document provenance score. In our
%% experiments we use provenance scores as features for the classifier.

\subsection{Eliminating Slot-Filler Aliases}
% comment by Vidh
% length, location, hierarchy of this section might change
% just putting it here for time being
When combining the output of different SF systems, it is possible that
some slot-filler entities might overlap with each other. An SF system
{\it A} could extract a filler {\it $F_1$} for a slot {\it S} while
another SF system {\it B} extracts another filler {\it $F_2$} for the
same slot {\it S}. If the extracted fillers $F_1$ and $F_2$ are {\it
  aliases} (i.e. different names for the same entity), the scoring
system for the TAC KBP SF task considers them redundant and
penalizes the precision of the system.

In order to eliminate aliases from the output of ensembled system, we
employ a technique derived by inverting the scheme used by the LSV SF
system \cite{roth:tac13} for query expansion. LSV SF uses a Wikipedia
anchor-text model \cite{roth:sigir10} to generate aliases for given
query entities. By including aliases for query names, the SF systems
increase the number of candidate sentences fetched for the query.

To eliminate filler aliases, we apply the same technique to generate
aliases for all slot fillers of a given query and slot type.  Given a
slot filler, we obtain the Wikipedia page that is most likely linked
to the filler text. Then, we obtain the anchor texts and their
respective counts from all other Wikipedia pages that link to this
page.  Using these counts, we choose top $N$ (we use $N$=10 as in LSV)
and pick the corresponding anchor texts as aliases for the given slot
filler. Using the generated aliases, we then verify if any of the slot
fillers are redundant with respect to these aliases. This scheme is
not applicable to slot types whose fillers are not entities (like
date or age). Therefore, simpler matching schemes are used to
eliminate redundancies for these slot types.


==> 2015/related_work.tex <==
Our system is part of a body of work on increasing the performance of relation
extraction through ensemble methods.

The use of {\it stacked generalization} for information extraction has been
demonstrated to outperform both majority voting and weighted voting methods
\cite{sigletos:jmlr05}.  In relation extraction, a stacked classifier
effectively combines a supervised, closed-domain Conditional Random Field-based
relation extractor with an open-domain CRF Open IE system, yielding a 10\%
increase in precision without harming recall \cite{banko:acl08}.  To our
knowledge, we are the first to apply stacking to KBP and the first to use
provenance as a feature in a stacking approach.

Many KBP SFV systems cast validation as a single-document problem and apply a
variety of techniques, such as rule based consistency checks
\cite{angeli:tac13}, and techniques from the well-known Recognizing Textual
Entailment (RTE) task \cite{cheng:tac13,sammons:tac14}.  In contrast, the 2013
{\it JHUAPL} system aggregates the results of many different extractors using a
constraint optimization framework, exploiting confidence values reported by each
input system \cite{wang:tac13}. A second approach in the {\it UI\_CCG} system
\cite{sammons:tac14} aggregates results of multiple systems by using majority
voting.

In the database, web-search, and data-mining communities, a line of research into ``truth-finding" or ``truth-discovery" methods addresses
the related problem of combining evidence for facts from multiple
sources, each with a latent credibility \cite{yin:kde08}.  The {\it
RPI\_BLENDER} KBP system
\cite{yu:coling14} casts SFV in this framework, using a graph propagation method
that modeled the credibility of systems, sources, and response
values. However they only report scores on the 2013 SFV data which
contain less complicated and easier queries compared to the 2014
data. Therefore, we cannot directly compare our system's performance to
their's.

Google's Knowledge Vault system \cite{dong:kdd14} combines the output of four
diverse extraction methods by building a boosted decision stump classifier
\cite{reyzin:ml2006}.  For each proposed fact, the classifier considers both the
confidence value of each extractor and the number of responsive documents found
by the extractor.  A separate classifier is trained for each predicate, and
Platt Scaling \cite{platt:book99} is used to calibrate confidence scores.

